Online Matching with Delays and Size-based Costs

In this paper, we introduce the problem of Online Matching with Delays and Size-based Costs (OMDSC). The OMDSC problem involves $m$ requests arriving online. At any time, a group can be formed by matching any number of these requests that have been received but are still unmatched. The cost associated with each group is determined by the waiting time for each request within the group and a size-dependent cost. Our goal is to partition all incoming requests into multiple groups while minimizing the total associated cost. The problem extends the TCP acknowledgment problem proposed by Dooly et al. (JACM 2001). It generalizes the cost model for sending acknowledgments. This paper reveals the competitive ratios for a fundamental case where the range of the penalty function is limited to $0$ and $1$. We classify such penalty functions into three distinct cases: (i) a fixed penalty of $1$ regardless of group size, (ii) a penalty of $0$ if and only if the group size is a multiple of a specific integer $k$, and (iii) other situations. The problem of case (i) is equivalent to the TCP acknowledgment problem, for which Dooly et al. proposed a $2$-competitive algorithm. For case (ii), we first show that natural algorithms that match all the remaining requests are $\Omega(\sqrt{k})$-competitive. We then propose an $O(\log k / \log \log k)$-competitive deterministic algorithm by carefully managing match size and timing, and we also prove its optimality. For case (iii), we demonstrate the non-existence of a competitive online algorithm. Additionally, we discuss competitive ratios for other typical penalty functions.

==> eng/chapters/discussion.tex <==
In this paper, we have clarified the competitive ratio for the OMDSC problem when the penalty functions take only values of either $0$ or $1$.
Let $\mu,\lambda\in\mathbb{R}$ with $0<\mu\le \lambda$, and consider a penalty function that takes values of $0$ or within the range $[\mu,\lambda]$. By applying our $\rho$-competitive algorithm to the problem, considering only whether the penalty is zero or $\mu$, we obtain a $(\rho\cdot \lambda/\mu)$-competitive algorithm. In addition, our impossibility can be transferred in the same way.
Another interesting penalty function would be $f(n) = \lceil n / k \rceil$ for a specific integer $k$.
This penalty function can be interpreted as a setting in a service that can process up to $k$ requests at once, where the penalty is determined based on the number of processing rounds.
For this penalty function, we can check that an algorithm, similar to the algorithm for (i), achieves a competitive ratio of $2$. However, it is unknown whether this competitive ratio can be improved.
% Consider any penalty function which takes the value of $0$. If the set of integers where the penalty function takes the value of $0$ does not coincide with the set of multiples of some integer $k$, we can prove that no online algorithm achieves a finite competitive ratio in the similar way to \Cref{thm:no_multiple}.

Furthermore, we propose examining a variant of the OMDSC problem that integrates a metric cost. Specifically, for $k = 2$ in case (ii), this problem is equivalent to the MPMDfp problem, proposed by Emek et al.~\cite{Emek2016-sa}. They demonstrated that the MPMDfp problem can be reduced to the MPMD problem by doubling the number of points in the metric space, even with multiple points. However, this approach of multiplying the number of points does not work for other penalty functions.
% $k > 2$, as it does for $k = 2$.
Exploring methodologies to overcome this difficulty is a valuable direction for future research.

% 本研究では, ペナルティ関数の値域が $0$ と $1$ のみからなる場合の OMDSC について競合比を明らかにした. 
% 他のペナルティ関数としては, ある整数 $k$ について, $f(n) = \lceil n / k \rceil$ となるようなものがある. このペナルティ関数は, 一度に最大 $k$ 個のリクエストを処理できるサービスにおいて, 処理を行う回数がペナルティになるような設定と考えられる. このペナルティ関数に対しては, (i) と似たアルゴリズムで競合比が $2$ 以下となることがわかっている. (要確認)
% 任意のペナルティ関数についても, ペナルティ関数が $0$ を取るような整数からなる集合が, ある整数 $k$ の倍数全体と一致しない場合は競合比が非有界になることも本論文の証明と同様に示すことができる.

% また, ペナルティ関数がある整数 $k$ の倍数のみ $0$, その他では $1$ を取るときの OMDSC 対して, 距離コストを導入することも考えられる. $k = 2$ のときは, Emek et al.~\cite{Emek2016-sa} らによって提案された MPMDfp と同じ問題である. MPMDfp は, single source でなくても, 距離空間上の点の数を $2$ 倍にした MPMD に帰着できることを彼らは示している. しかし, $k > 2$ については, 同様に距離空間の点の数を $k$ 倍するだけではうまくいかない. 

==> eng/proofs/Bf_empty.tex <==
In this section, we explore the case where $B_f = \emptyset$, indicating that $f(x)=1$ for any positive integer $x \in \mathbb{Z}_{++}$.
%the cost to match $x$ requests at once is $1$ for any positive integer $x \in \mathbb{Z}_{++}$.
We propose a deterministic online algorithm for the penalty function and show that its competitive ratio is $2$. Moreover, we demonstrate that this competitive ratio is best possible.

% $B_f = \emptyset$ である場合, 任意の整数 $x \in \mathbb{Z}_{++}$ について $x$ 個のリクエストを一度にマッチするコストは $1$ である. このようなペナルティ関数に対して決定的オンラインアルゴリズムを提案し, その競合比が $2$ であることを示す. そして, 任意の決定的オンラインアルゴリズムについて, 競合比が $2$ 以上となることを示す. 

\subsection{Upper Bound}
We first provide a $2$-competitive algorithm.
\begin{theorem} \label{thm:all_1}
    When the penalty function $f$ satisfies $B_f = \emptyset$, the OMDSC problem admits a deterministic online algorithm with a competitive ratio of at most $2$.
\end{theorem}

% \begin{thm} \label{thm:all_1}
%     ペナルティ関数 $f$ に対して $B_f = \emptyset$ であるとき, 競合比が $2$ 以下である決定的オンラインアルゴリズムが存在する. 
% \end{thm}

\begin{proof}
    We propose a deterministic online algorithm, denoted as $\ALG$. 
    For any instance $\sigma$, let $m_\sigma$ represent the number of matches made by $\ALG$, 
     and let $\tau_i$ denote the time of the $i$th match is made, where $\tau_0 \coloneqq 0 < \tau_1 < \tau_2 < \cdots < \tau_{m_\sigma}$.
    Furthermore, we use $\ALG(\sigma)$ and $\OPT(\sigma)$ to denote the costs incurred by $\ALG$ and an optimal offline algorithm $\OPT$, respectively.
    We aim to demonstrate that $\ALG(\sigma)$ is $2m_\sigma$, and $\OPT(\sigma)$ is at least $m_\sigma$, resulting in a competitive ratio of $2$.

    The algorithm $\ALG$ matches all remaining requests once the waiting cost reaches $1$. Specifically, let $r$ denote the number of requests that have been presented but remain unmatched, and the algorithm maintains a variable $w$ that increases at the same rate as the waiting cost. 
    Here, $w$ is a continuous variable with $\dv*{w}{t} = r$.
    The algorithm matches all remaining requests when $w = 1$ and then resets $w$ to $0$. Thus, each match incurs a total cost of $2$: $1$ for the size cost and $1$ for the waiting cost.
    %For any instance $\sigma$, let $m_\sigma$ be the number of matches made by the algorithm, and let $\tau_i$ denote the time of the $i$-th match, with $\tau_0 \coloneqq 0 < \tau_1 < \tau_2 < \cdots < \tau_{m_\sigma}$.
    %Since each match incurs a cost of $2$, 
    Consequently, the total cost for $\sigma$ is $2m_\sigma$.

    Next, we provide a lower bound for the cost of the optimal offline algorithm. For all $i \in \{0, 1, \ldots, m_\sigma-1\}$, we show that a cost of at least $1$ is incurred during the interval of $(\tau_{i}, \tau_{i + 1}]$.
    To analyze this, we denote the values of $w$ and $r$ at time $t$ by $w(t)$ and $r(t)$, respectively. If a match occurs at time $t$, we take the values right after the match.
    If the optimal offline algorithm makes a match in the interval of $(\tau_i,\tau_{i + 1}]$, a match cost of $1$ is incurred. 
    Otherwise (i.e., no match is made in the interval of $(\tau_{i},\tau_{i + 1}]$), suppose that the algorithm has $r'~(\ge 0)$ leftover requests right after $\tau_i$. % while $r(\tau_i) = 0$.
    Given that $\ALG$'s waiting cost is $1$ during this time interval, $\OPT$'s waiting cost is at least
    $\int_{\tau_i}^{\tau_{i + 1}} r' + r(t) \dd{t} \geq \int_{\tau_i}^{\tau_{i+1}} r(t) \dd{t} = \int_{\tau_i}^{\tau_{i+1}} \dv{w(t)}{t} \dd{t} = 1$,
    implying that a cost of at least $1$ is incurred in either case. Thus, the total cost of $\OPT$ for the entire instance is at least $m_\sigma$.

    Therefore, as $\ALG(\sigma) = 2m_{\sigma}$ and $\OPT(\sigma) \geq m_{\sigma}$, the competitive ratio is at most $2$.
\end{proof}

% \begin{proof}
% 決定的オンラインアルゴリズムを提案し, 任意のインスタンス $\sigma$ に対して, そのオンラインアルゴリズムがマッチを行う回数を $m$ とおく. その後, $\sigma$ に対するオンラインアルゴリズムのコストが $2m$, 最適オフラインアルゴリズムのコストが $m$ 以上であることを示し, 競合比が $2$ であることを導く. 

% 我々が提案するオンラインアルゴリズムは, 待機コストが $1$ かかる度に余っているリクエストをすべてマッチする. 詳細には, 既に与えられたリクエストの内, まだマッチしていないリクエストの個数を $r$ とし, アルゴリズムは待機コストと同じ速さで増加する変数 $w$ を持つ. ここで, $w$ は連続的な変数であって, $\dv*{w}{t} = r$ である. アルゴリズムは, $w = 1$ になると同時に余っているリクエストをすべてマッチさせ, $w = 0$ に初期化する. このオンラインアルゴリズムはマッチの度にマッチコスト $1$ と待機コスト $1$ の合計 $2$ がコストとしてかかる.

% 任意のインスタンスに対して, そのインスタンスで提案アルゴリズムがマッチする回数を $m$, $i$ 回目にマッチを行った時刻 $\tau_i$ とし, $\tau_0 \coloneqq 0 < \tau_1 < \tau_2 < \cdots < \tau_m$ を仮定する. このとき, 各マッチごとにコストが $2$ かかるため, インスタンス全体でのコストは $2m$ となる.

% 次に, 最適オフラインアルゴリズムのコストを下から抑える. そのために, すべての $i \in \{0, 1, \ldots, m - 1\}$ について, 時刻 $\tau_i$ の直後から 時刻 $\tau_{i + 1}$ までの間に $1$ 以上のコストがかかることを示す. 解析のために, 時刻 $t$ での提案アルゴリズムの $w$ と $r$ の値をそれぞれ $w(t), r(t)$ と表す. ただし, 時刻 $t$ で提案アルゴリズムがマッチを行う場合, マッチを行った直後の値を表す. 

% まず, 最適オフラインアルゴリズムが時刻 $\tau_i$ の直後から時刻 $\tau_{i + 1}$ までの間にマッチを行う場合, そこでマッチコスト $1$ がかかる. そうでないとき, 時刻 $\tau_i$ から $\tau_{i + 1}$ までの間にマッチを行わない. このとき, 時刻 $\tau_i$ の直後で最適オフラインアルゴリズムは $r'$ 個のリクエストを余らせている. 一方, $r(\tau_i) = 0$ である. この時刻間でのオンラインアルゴリズムの待機コストが $1$ であることから, 最適オフラインアルゴリズムの待機コストは, 
% \[
%     \int_{\tau_i}^{\tau_{i + 1}} r' + r(t) \dd{t} \geq \int_{\tau_i}^{\tau_{i+1}} r(t) \dd{t} = \int_{\tau_i}^{\tau_{i+1}} \dv{w(t)}{t} \dd{t} = 1
% \]
% より $1$ 以上である. よって, いずれの場合も $1$ 以上のコストがかかり, インスタンス全体では $m$ 以上のコストがかかる. 

% したがって, 提案アルゴリズムがマッチした回数を $m$ としたとき, 提案アルゴリズムのコストは $2m$, 最適オフラインアルゴリズムのコストは $m$ 以上である. このことから, 競合比は $2$ 以下である.
% \end{proof}


\subsection{Lower Bound}
Next, we establish a lower bound for the competitive ratio of any online algorithm $\ALG$. We first describe the construction of an instance $\sigma_{\ALG}^{M,n}$ against the online algorithm $\ALG$ with parameters $n\in\mathbb{Z}_{+}$ and $M\in\mathbb{Z}_{++}$, and then evaluate the cost for $\ALG$ and the optimal offline algorithm $\OPT$ on $\sigma_{\ALG}^{M,n}$.
We will demonstrate that, for any $\varepsilon>0$, there exist some parameters $n$ and $M$ such that the competitive ratio of $\ALG$ for $\sigma_{\ALG}^{M,n}$ is at least $2-\varepsilon$.

% 次に, 任意のオンラインアルゴリズムの競合比を下から抑える. まず, オンラインアルゴリズム $\mathcal{ALG}$ に対するインスタンス $\sigma_{\mathcal{ALG}}^M$ の構成方法を説明する. その後, $\sigma_{\mathcal{ALG}}^M$ に対する $\mathcal{ALG}$ と最適オフラインアルゴリズムのコストを抑える. 

\begin{theorem} \label{thm:all_1_lower}
    When the penalty function $f$ satisfies $B_f = \emptyset$, the OMDSC problem admits no deterministic online algorithm with a competitive ratio of strictly less than $2$. %can achieve a competitive ratio less than $2 - \varepsilon$ for any $\varepsilon > 0$.
\end{theorem}

% \begin{thm} \label{thm:all_1_lower}
%     ペナルティ関数 $f$ に対して $B_f = \emptyset$ であるとき, 任意の $\varepsilon > 0$ について, 競合比 $2 - \varepsilon$ 未満となるオンラインアルゴリズムは存在しない. 
% \end{thm}

The instance $\sigma_{\ALG}^{M,n}$ consists of $\sum_{i=0}^{n}M^{2i}$ requests.
The first request appears at time $0$.
Subsequently, for each $i\in\{1,2,\dots,n\}$, 
$M^{2i}$ requests are presented right after the $i$th match is executed by $\ALG$.
We assume, without loss of generality, that $\ALG$ matches all the requests within a finite time for any instance of the form $\sigma_{\ALG}^{M,n}$. 
If this assumption does not hold, the competitive ratio of $\ALG$ becomes infinite.
For $i\in\mathbb{Z}_{++}$, let $\tau_{M,i}$ be the time such that $\ALG$ makes $i$th match for $\sigma^{M,n}_{\ALG}$ with $n\ge i-1$.
Additionally, for $i\in\mathbb{Z}_+$, we define $\delta_{M,i}$ to be $\tau_{M,i+1}-\tau_{M,i}$, where we assume $\tau_{M,0}=0$.
%For any online algorithm $\ALG$, in an instance, one request is given at the start, then for a sufficiently large integer $M \gg 0$, $M^{2i}$ requests are given right after the $i$th match performed by $\ALG$.
%Here, for any $n \in \mathbb{Z}_+$, if $\ALG$ performs $n$ or more matches, the instance composed of requests up to the $(n + 1)$-th given is denoted by $\sigma_{\ALG}^{M, n+1}$.
%Moreover, for some $n \in \mathbb{Z}_+$ where the number of matches by $\ALG$, the instance ends when the $(n + 1)$-th requests are given. 
% In detail, the instance $\sigma^M_{\ALG}$ is constructed as follows:
% \begin{description}
% \setlength{\itemsep}{6pt}
%     \item[At the start:] \,\\
%         Keep track of the number of giving requests, $n$. Initially, give one request at time $0$ and set $n = 1$.

%     \item[When $\ALG$ performs a match:] \,\\
%         Let the elapsed time since the last request was given as $\delta_{n - 1}$. Right after the match, give $M^{2n}$ requests and increase $n$ by $1$.
% \end{description}

% 任意のオンラインアルゴリズム $\mathcal{ALG}$ に対するインスタンスでは, 開始直後に $1$ つのリクエストが与えられた後, 十分大きい整数 $M \gg 0$ について, $\mathcal{ALG}$ が $i$ 回目のマッチを行った直後に $M^i$ 個のリクエストが与えられる.
% ここで, 任意の $n \in \mathbb{Z}_+$ について, $\mathcal{ALG}$ が $n$ 回以上マッチを行うとき, $n + 1$ 回目に与えられるリクエストまでからなるインスタンスを $\sigma_{\mathcal{ALG}}^{M, n + 1}$ と表す.
% また, ある $n \in \mathbb{Z}_+$ について, $\mathcal{ALG}$ がマッチを行う回数が $n$ である場合, インスタンスは $n + 1$ 回目にリクエストが与えられた時点で終了する. 
% 詳細には, 次のようにインスタンス $\sigma_{\mathcal{ALG}}^M$ を構成する. 

% \begin{description}
% \setlength{\itemsep}{6pt}
%     \item[開始時] \,\\
%         十分大きな整数 $M \in \mathbb{Z}_{++}$ を取り, リクエストを与えた回数 $n$ を持つ. まず, 時刻 $0$ に $1$ つのリクエストを与え, $n = 1$ とする. 

%     \item[$\mathcal{ALG}$ がリクエストをマッチしたとき] \,\\
%         最後にリクエストを与えてからの (elapsed time) 経過時間を $\delta_{n - 1}$ とする. マッチ直後, $M^{2n}$ 個のリクエストを与え, $n$ を $1$ 増やす. 
% \end{description}
% \noindent
% This construction of $\sigma_{\ALG}^M$ does not guarantee that the number of given requests is finite. However, for any $\varepsilon > 0$, we show that there exists some $n \in \mathbb{Z}_{++}$ where the cost ratio for $\sigma_{\ALG}^{M, n}$ is at least $2 - \varepsilon$.
% このようにして構成した $\sigma_{\mathcal{ALG}}^M$ では, リクエストを与えられる回数が有限とは限らない. しかし, 任意の $\varepsilon > 0$ について, ある $n \in \mathbb{Z}_{++}$ が存在し, $\sigma_{\mathcal{ALG}}^{M, n}$ に対するコストの比が $2 - \varepsilon$ 以上であることを示す. 

In the proof, we first bound $\ALG\left(\sigma_{\ALG}^{M, n}\right)$ and $\OPT\left(\sigma_{\ALG}^{M, n}\right)$ for any $n \in \mathbb{Z}_+$, respectively. Then, depending on the values of $\OPT\left(\sigma_{\ALG}^{M, n}\right)$ for all $n \in \mathbb{Z}_{+}$, we evaluate the competitive ratio by case division.
% まず, $\mathcal{ALG}$ と最適オフラインアルゴリズムのコストをそれぞれ下と上から抑える. その後, $\sigma_{\mathcal{ALG}}^M$ で与えられるリクエストが有限かどうかと最適オフラインアルゴリズムの $\sigma_{\mathcal{ALG}}^{M, n}$ に対するコストで場合分けを行い, 競合比を評価する.

\begin{lemma} \label{lmm:all_1_cost}
    For any deterministic online algorithm $\ALG$ with the instance $\sigma_{\ALG}^{M,n}$, we have
    \begin{align*}
        \ALG\left(\sigma_{\ALG}^{M, n}\right) \geq \sum_{i = 0}^{n} \left(1 + M^{2i} \cdot \delta_{M,i}\right)
        \ \text{and}\ 
        \OPT\left(\sigma_{\ALG}^{M, n}\right) \leq 1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i=0}^{n - 1} M^{2i} \cdot \delta_{M,i}. 
    \end{align*}
\end{lemma}

% \begin{lem} \label{lmm:all_1_cost}
%     任意のオンラインアルゴリズム $\mathcal{ALG}$ に対して, インスタンス $\sigma_{\mathcal{ALG}}^M$ を取る. 任意の $n \in \mathbb{Z}_{++}$ について, $\sigma_{\mathcal{ALG}}^{M, n}$ が存在するとき, $\sigma_{\mathcal{ALG}}^{M, n}$ に対する $\mathcal{ALG}$ のコストは, 
%     \[
%         \sum_{i = 0}^{n - 1} \left(1 + M^{2i} \cdot e_i\right)
%     \]
%     以上であり, 最適オフラインアルゴリズムのコストは,
%     \[
%         1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i=0}^{n - 2} M^{2i} \cdot e_i
%     \]
%     以下である. 
% \end{lem}

\begin{proof}
    %From the construction of $\sigma_{\ALG}^{M, n}$, for any $i \in \mathbb{Z}_n$, $\ALG$ matches $M^{2i}$ requests after time $e_i$ has elapsed. Considering an online algorithm that matches all remaining requests without loss, the cost consists of a match cost of $1$ and a waiting cost of $M^{2i} \cdot e_i$ for each match. 
    By the definition of $\sigma_{\ALG}^{M,n}$, the total cost is 
    $\ALG\left(\sigma_{\ALG}^{M, n}\right) \geq \sum_{i = 0}^{n} \left(1 + M^{2i}\cdot  \delta_{M, i}\right)$.
    To bound the cost of the optimal offline algorithm, we consider an algorithm that matches all the given requests at the time when the last request is given. 
    %Unlike $\ALG$, it matches right after $n$-th requests are given. When $M \geq 2$, for any $l \in \mathbb{Z}_{++}$,
    Then, the total cost of $\OPT$ can be bounded as
    \begin{align}
        \OPT\left(\sigma_{\ALG}^{M, n}\right) 
        &\leq 1 + \sum_{i = 0}^{n-1} \Big(\delta_{M,i} \cdot \sum_{j = 0}^{i} M^{2j} \Big) 
        \leq 1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i = 0}^{n - 1} (M^{2i} \cdot \delta_{M,i}),
    \end{align}
    where the second inequality holds by $\sum_{j = 0}^{i} M^{2j} = \frac{M^{2(i+1)}-1}{M^2-1} \leq \frac{M^2}{M^{2} - 1} \cdot M^{2i}$.
\end{proof}

% \begin{proof}
%     インスタンス $\sigma_{\mathcal{ALG}}^{M, n}$ の構成から, 任意の $i \in \mathbb{Z}_{n}$ に対して $\mathcal{ALG}$ は $i + 1$ 回目に与えられた $M^{2i}$ 個のリクエストを時間が $e_i$ 経過した後にマッチする. ここで, 与えられているリクエストをすべてマッチしても損をしないため, すべてをマッチするオンラインアルゴリズムのコストを考える. このとき, マッチコスト $1$ と待機コスト $M^{2i} \cdot e_i$ がかかる. よって, 合計コストは
%     \[
%         \sum_{i = 0}^{n - 1} \left(1 + M^{2i}\cdot  e_i\right)
%     \]
%     以上となる. 
%     オフラインアルゴリズムのコストとしては, 途中でマッチを行わず, $n$ 回分のリクエストをまとめてマッチするときのコストを考える. このとき, $\mathcal{ALG}$ とは異なり, 最後に $M^{2(n - 1)}$ 個のリクエストが与えられた直後にマッチを行う. $M \geq 2$ のとき, 任意の $l \in \mathbb{Z}_{+}$ に対して, 
%     \[
%         \sum_{i = 0}^{l} M^{2i} \leq \frac{M^2}{M^{2} - 1} \cdot M^{2l}
%     \]
%     であることから, 最適オフラインアルゴリズムのコストは
%     \[
%         1 + \sum_{i = 0}^{n - 2} \left(e_i \cdot \sum_{j = 0}^{i} M^{2j} \right) \leq 1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i = 0}^{n - 2} M^{2i} \cdot e_i
%     \]
%     以下となる.
% \end{proof}

We perform the competitive analysis in two cases, according to whether the value $\frac{M^2}{M^2 - 1}\left(\sum_{i = 0}^{n-1} M^{2i} \cdot \delta_{M,i}\right)$ exceeds $n$ for any $n\ge 1$.
%three cases based on the instance $\sigma_{\ALG}^M$:
% \begin{itemize}
% \item The number of requests given in $\sigma_{\ALG}^M$ is finite,

% \item For some integer $n \geq 2$, $\OPT\left(\sigma_{\ALG}^{M, n}\right) > n$,

% \item For any integer $n \geq 2$, $\OPT\left(\sigma_{\ALG}^{M, n}\right) \leq n$.
% \end{itemize}

% 競合比を評価するために, 
% \begin{itemize}
% \item $\sigma_{\mathcal{ALG}}^M$ でリクエストを与えられる回数が有限

% \item ある $2$ 以上の整数 $n$ について, $\sigma_{\mathcal{ALG}}^{M, n}$ に対する最適オフラインアルゴリズムのコストが $n$ より大きい

% \item 任意の $2$ 以上の整数 $n$ について, $\sigma_{\mathcal{ALG}}^{M, n}$ に対する最適オフラインアルゴリズムのコストが $n$ 以下
% \end{itemize}
% の $3$ 通りに場合分けを行い, それぞれについてコスト比を評価する. 


% \begin{lem} \label{lmm:all_1_finite}
%     If the number of requests given in $\sigma_{\ALG}^M$ is finite, then the cost ratio between $\ALG$ and $\OPT$ for $\sigma_{\ALG}^M$ is at least $2$.
% \end{lem}

% \begin{proof}
%     Let the number of times requests have been given as $n$, not the number of given requests. Since $e_i$ for each $i \leq n - 2$ is finite, $\OPT\left(\sigma_{\ALG}^M\right)$ can be bounded by
%     \[
%     C \coloneqq 1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i=0}^{n -2} M^{2i} \cdot e_i.
%     \]
%     Meanwhile, $\ALG$ waits more than $2C$ time without matching $M^{2(n - 1)}$ requests given last. Thus, the cost of $\ALG$ is at least $2C \cdot M^{2(n - 1)}$, leading to a cost ratio of at least $2$.
% \end{proof}

% \begin{lem} \label{lmm:all_1_finite}
%     $\sigma_{\mathcal{ALG}}^M$ でリクエストを与えられる回数が有限であるとき, $\sigma_{\mathcal{ALG}}^M$ に対する $\mathcal{ALG}$ と最適オフラインアルゴリズムのコスト比は $2$ 以上である. 
% \end{lem}

% \begin{proof}
%     $\sigma_{\mathcal{ALG}}^M$ でリクエストが与えられる回数を $n$ とする. $n - 2$ 以下の任意の整数 $i$ について $e_i$ は有限であることから, $\sigma_{\mathcal{ALG}}^M$ に対する
%     最適オフラインアルゴリズムのコストは, 
%     \[
%     C \coloneqq 1 + \frac{M^2}{M^2 - 1} \cdot \sum_{i=0}^{n -2} M^{2i} \cdot e_i
%     \]
%     以下より有限である. 一方で, $\sigma_{\mathcal{ALG}}^M$ に対して $\mathcal{ALG}$ は $M^{2(n - 1)}$ 個のリクエストをマッチしないまま $2C$ 以上の時間を待機する. よって, $\mathcal{ALG}$ のコストは, $2C\cdot M^{2(n - 1)}$ 以上である. 

%     したがって, コスト比は $2$ 以上である.
% \end{proof}

\begin{lemma} \label{lmm:all_1_exist_nstar}
    %For the instance $\sigma_{\ALG}^{M,n}$, 
    Suppose that there exists an integer $n \geq 1$ such that
    $\frac{M^2}{M^2 - 1}\big(\sum_{i = 0}^{n-1} M^{2i} \cdot \delta_{M,i}\big) > n$
    and let $n^*$ be the smallest such $n$. Then, the competitive ratio for $\sigma_{\ALG}^{M, n^* - 1}$ is at least $1 + (M^2 - 1) / M^2$.
\end{lemma}

\begin{proof}
    %The left hand side of the inequality \eqref{ineq:over_n} represents an upper bound for $\OPT\left(\sigma_{\ALG}^{M, n}\right)$ by Lemma~\ref{lmm:all_1_cost}. 
    We consider cases for $n^* = 1$ and $n^* \geq 2$, showing that the cost ratios meet the specified bound in both cases.

    When $n^* = 1$, we have $\frac{M^2}{M^2 - 1} \cdot \delta_{M,0} > 1$.
    Then, we have $\ALG\left(\sigma_{\ALG}^{M, 0}\right) = 1 + \delta_{M,0} > 1 + \frac{M^2 - 1}{M^2}$.
    Hence, $\ALG\left(\sigma^{M,0}_{\ALG}\right)/\OPT\left(\sigma^{M,0}_{\ALG}\right)$ is at least $1 + (M^2 - 1) / M^2$ by $\OPT\left(\sigma_{\ALG}^{M, 0}\right)=1$.

    For the case of $n^* \geq 2$, %since $n^*$ is the smallest integer satisfying inequality \eqref{ineq:over_n}, 
    we have
    \begin{align*}
    \textstyle
        \frac{M^2}{M^2 - 1} \cdot \left(\sum_{i = 0}^{n^* - 1} M^{2i} \cdot \delta_{M,i} \right) > n^* \quad\text{and}\quad
        \frac{M^2}{M^2 - 1} \cdot \left(\sum_{i = 0}^{n^* - 2} M^{2i} \cdot \delta_{M,i} \right) \leq n^* - 1.
    \end{align*}
    Therefore, $\OPT(\sigma_{\ALG}^{M, n^*-1})\le 1+\frac{M^2}{M^2 - 1} \cdot \left(\sum_{i = 0}^{n^*-2} M^{2i} \cdot \delta_{M,i} \right)\le n^*$ and 
    \[
    \textstyle
        \ALG(\sigma_{\ALG}^{M, n^*-1})
        \ge\sum_{i=0}^{n^*-1} \left(1+M^{2i} \cdot \delta_{M,i}\right) 
        > n^*+ \frac{M^2 - 1}{M^2} \cdot n^*
    \]
    by \Cref{lmm:all_1_cost}.
    Thus, $\ALG\left(\sigma^{M,n^*-1}_{\ALG}\right)/\OPT\left(\sigma^{M,n^*-1}_{\ALG}\right)$ is greater than $1 + (M^2 - 1) / M^2$.
    %Consequently, the cost ratio between $\OPT$ and $\ALG$ for $\sigma_{\ALG}^{M, n^* - 1}$ is at least $1 + (M^2 - 1) / M^2$.
\end{proof}

% \begin{lem} \label{lmm:all_1_exist_nstar}
%     $\sigma_{\mathcal{ALG}}^M$ について, ある $2$ 以上の整数 $n$ として
%     \begin{equation}
%         1 + \frac{M^2}{M^2 - 1}\left(\sum_{i = 0}^{n-2} M^{2i} \cdot e_i\right) > n  \label{ineq:over_n}
%     \end{equation}
%     を満たすものが存在するとき, その最小値を $n^*$ とする. すると, $\sigma_{\mathcal{ALG}}^{M, n^*-1}$ に対する $\mathcal{ALG}$ と最適オフラインアルゴリズムのコスト比は $1 + (M^2 - 1) / M^2$ 以上である.
% \end{lem}

% \begin{proof}
%     不等式 \eqref{ineq:over_n} の左辺は, Lemma \ref{lmm:all_1_cost} より $\sigma_{\mathcal{ALG}}^{M, n}$ に対する最適オフラインアルゴリズムのコストの上界である. $n^* = 2$ と $n^* \geq 3$ で場合分けをして示す.
    
%     $n^* = 2$ のとき, 
%     \[
%         1 + \frac{M^2}{M^2 - 1} \cdot t_0 > 2
%     \]
%     である. よって, $\sigma_{\mathcal{ALG}}^{M, n^*-1}$ に対する最適オフラインアルゴリズムのコストは $1$, $\mathcal{ALG}$ のコストについては
%     \[
%         1 + \sum_{i = 0}^{n^* - 2} \left(M^{2i} \cdot t_i\right) = 1 + t_0 > 1 + \frac{M^2 - 1}{M^2}
%     \]
%     が成り立つ. よって, コストの比は $1 + (M^2 - 1) / M^2$ 以上である.

%     $n^* \geq 3$ の場合を考える. 
%     不等式 \eqref{ineq:over_n} を満たす整数の中で $n^*$ は最小であることから, 
%     \begin{align*}
%         1 + \frac{M^2}{M^2 - 1} \cdot \left(\sum_{i = 0}^{n^* - 2} M^{2i} \cdot t_i \right) &> n^*, \\
%         1 + \frac{M^2}{M^2 - 1} \cdot \left(\sum_{i = 0}^{n^* - 3} M^{2i} \cdot t_i \right) &\leq n^* - 1
%     \end{align*}
%     が成り立つ. よって, $\sigma_{\mathcal{ALG}}^{M, n^*-1}$ に対する最適オフラインアルゴリズムのコストは $n^* - 1$ 以下である. $\mathcal{ALG}$ のコストについては, 
%     \[
%         (n^* - 1) + \sum_{i=0}^{n^*-2} \left(M^{2i} \cdot t_i\right) 
%         > (n^* - 1) + \frac{M^2 - 1}{M^2} \cdot (n^* - 1)
%     \]
%     が成り立つ. よって, コストの比は $1 + (M^2 - 1) / M^2$ 以上である.

%     したがって, $\sigma_{\mathcal{ALG}}^{M, n^*-1}$ に対する最適オフラインアルゴリズムと $\mathcal{ALG}$ のコスト比は $1 + (M^2 - 1) / M^2$ 以上である.
% \end{proof}

\begin{lemma} \label{lmm:all_1_no_exist}
    For an integer $n\ge 1$, if $\frac{M^2}{M^2 - 1}\left(\sum_{i=0}^{n - 1} M^{2i} \cdot \delta_{M,i}\right) \leq n$, then we have $\ALG(\sigma_{\ALG}^{M, n})/\OPT(\sigma_{\ALG}^{M,n})\ge \frac{n}{n+1} + \frac{M^2 - 1}{M^2}$.
\end{lemma}
\begin{proof}
    % Given inequality \eqref{ineq:below_n} and \Cref{lmm:all_1_cost}, the cost of $\OPT$ is less than or equal to $n$.
    % Therefore, we can evaluate the cost ratio by bounding the cost for $\ALG$ by the cost for $\OPT$.
    By Lemma \ref{lmm:all_1_cost}, we have
    \begin{align*}
        \ALG\left(\sigma_{\ALG}^{M, n}\right) 
        \ge \sum_{i=0}^{n} \left(1+M^{2i} \cdot \delta_{M,i}\right)  
        &\geq n + \tfrac{M^2 - 1}{M^2} + \tfrac{M^2 - 1}{M^2} \cdot \tfrac{M^2}{M^2 - 1} \cdot \sum_{i = 0}^{n - 1} \left(M^{2i} \cdot \delta_{M,i} \right) \\
        &\geq n + \tfrac{M^2 - 1}{M^2} \cdot \OPT\left(\sigma_{\ALG}^{M, n}\right).
    \end{align*}
    Combining this with $\OPT(\sigma_{\ALG}^{M, n})\le  1+\frac{M^2}{M^2 - 1}\left(\sum_{i=0}^{n - 1} M^{2i} \cdot \delta_{M,i}\right) \leq n+1$, we obtain
    \[
    \textstyle
        \frac{\ALG\left(\sigma_{\ALG}^{M, n}\right)}{\OPT\left(\sigma_{\ALG}^{M, n}\right)} 
        \geq \frac{n}{\OPT\left(\sigma_{\ALG}^{M, n}\right)} + \frac{M^2 - 1}{M^2}
        \geq \frac{n}{n+1} + \frac{M^2 - 1}{M^2},
    \]
    which proves the lemma.
\end{proof}


% \begin{lem} \label{lmm:all_1_no_exist}
%     $\sigma_{\mathcal{ALG}}^M$ について, 任意の $2$ 以上の整数 $n$ に対して
%     \begin{equation}
%         1 + \frac{M^2}{M^2 - 1}\left(\sum_{i=0}^{n - 2} M^{2i} \cdot t_i\right) \leq n \label{ineq:below_n}
%     \end{equation}
%     が成り立つとする. このとき, 任意の $2$ 以上の整数 $n$ について, $\sigma_{\mathcal{ALG}}^{M, n}$ に対する最適オフラインアルゴリズムと $\mathcal{ALG}$ のコスト比は, 
%     \[
%         \frac{n-1}{n} + \frac{M^2 - 1}{M^2}
%     \]
%     以上である.
% \end{lem}

% \begin{proof}
%     不等式 \eqref{ineq:below_n} と Lemma \ref{lmm:all_1_cost} より, 最適オフラインアルゴリズムのコストは $n$ 以下である. よって, $\mathcal{ALG}$ のコストを最適オフラインアルゴリズムのコストを用いて下から抑える.
    
%     $\sigma_{\mathcal{ALG}}^{M, n}$ に対する最適オフラインアルゴリズムのコストを $OPT$, $\mathcal{ALG}$ のコストを $ALG$ とすると, 
%     \begin{align*}
%         ALG &= n + \sum_{i=0}^{n - 1} \left(M^{2i} \cdot t_i\right)  \\
%         &\geq (n - 1) + \frac{M^2 - 1}{M^2} + \frac{M^2 - 1}{M^2} \cdot \frac{M^2}{M^2 - 1} \cdot \sum_{i = 0}^{n - 2} \left(M^{2i} \cdot t_i \right) \\
%         &= (n - 1) + \frac{M^2 - 1}{M^2} \cdot OPT
%     \end{align*}
%     となる. よって, $OPT \leq n$ と合わせて, 
%     \[
%         \frac{ALG}{OPT} \geq \frac{n - 1}{n} + \frac{M^2 - 1}{M^2}
%     \]
%     が成り立つ.
% \end{proof}

Now, we are ready to prove \Cref{thm:all_1_lower}.
\begin{proof}[Proof of \Cref{thm:all_1_lower}]
    Fix $\varepsilon > 0$ and an online algorithm $\ALG$.
    We prove that the competitive ratio of $\ALG$ for $\sigma_{\ALG}^{M,n}$ is at least $2-\epsilon$ for some $M$ and $n$.
    % For any online algorithm $\ALG$, we construct the instance $\sigma_{\ALG}^M$ based on $\ALG$'s processing.
    % Then, we evaluate the costs of $\ALG$ and $\OPT$ for $\sigma_{\ALG}^M$ to demonstrate the competitive ratio.
    %
    %For any online algorithm $\ALG$, once an integer $M$ is determined, we can construct $\sigma_{\ALG}^M$.
    %If the number of requests provided in $\sigma_{\ALG}^M$ is finite, Lemma \ref{lmm:all_1_finite} ensures that the competitive ratio is at least $2$.
    %Therefore, we consider the case where the number of requests provided is infinite. In this case, either the assumption of Lemma \ref{lmm:all_1_exist_nstar} or Lemma \ref{lmm:all_1_no_exist} holds for $\sigma_{\ALG}^M$.
    %For each case, we show that choosing sufficiently large $M$ and $n$ yields a competitive ratio greater than or equal to $2 - \varepsilon$.
    We set $M=\lceil\sqrt{2/\varepsilon}\rceil$. Note that we have $1 / M^2 < \varepsilon / 2$.
    %Firstly, we select $M$ such that $1 / M^2 < \varepsilon / 2$ and construct $\sigma_{\ALG}^M$.
    %
    If $\frac{M^2}{M^2 - 1}\left(\sum_{i = 0}^{n-1} M^{2i} \cdot \delta_{M,i}\right) > n$ for some $n\ge 1$, 
    % When the assumption of Lemma \ref{lmm:all_1_exist_nstar} holds, 
    then we take the minimum such integer $n^*$ as defined in \Cref{lmm:all_1_exist_nstar}. Then, the competitive ratio of $\ALG$ for $\sigma_{\ALG}^{M, n^* - 1}$ is at least
    $1 + \frac{M^2 - 1}{M^2} = 2 - \frac{1}{M^2} > 2 - \varepsilon$.
    %
    If $\frac{M^2}{M^2 - 1}\left(\sum_{i = 0}^{n-1} M^{2i} \cdot \delta_{M,i}\right) \le n$ for any $n\ge 1$, 
    the competitive ratio of $\ALG$ for $\sigma_{\ALG}^{M, M^2-1}$ is at least
    $\frac{M^2 - 1}{M^2} + \frac{M^2 - 1}{M^2} = 2-\frac{2}{M^2} > 2-\varepsilon$.
    % Therefore, by choosing $n'$ such that $1 / n' < \varepsilon / 2$, the cost ratio for $\sigma_{\ALG}^{M, n'}$ becomes:
    % \[
    %     \frac{n' - 1}{n'} + \frac{M^2 - 1}{M^2} = 2 - \frac{1}{n'} - \frac{M^2 - 1}{M^2} > 2 - \varepsilon.
    % \]

    Thus, for any online algorithm and any $\varepsilon > 0$, the competitive ratio is at least $2 - \varepsilon$.
\end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:all_1_lower}]
%     $\varepsilon > 0$ を固定する.
%     任意のオンラインアルゴリズム $\mathcal{ALG}$ に対して, その処理に応じてインスタンス $\sigma_{\mathcal{ALG}}^M$ を構成する. その後, $\sigma_{\mathcal{ALG}}^M$ に対する $\mathcal{ALG}$ と最適オフラインアルゴリズムのコストを評価して競合比を示す. 

%     任意のオンラインアルゴリズム $\mathcal{ALG}$ に対して, 整数 $M$ を決めると $\sigma_{\mathcal{ALG}}^M$ が構成できる.
%     $\sigma_{\mathcal{ALG}}^M$ でリクエストを与えられる回数が有限であるとき, Lemma \ref{lmm:all_1_finite} より競合比は $2$ 以上である. 
%     よって, リクエストを与えられる回数が有限でない場合を考える.
%     このとき, インスタンス $\sigma_{\mathcal{ALG}}^M$ に対して, Lemma \ref{lmm:all_1_exist_nstar} もしくは Lemma \ref{lmm:all_1_no_exist} のどちらか一方の仮定が成り立つ. それぞれについて, 十分大きい $M$ と $n$ を取ると, 競合比が $2 - \varepsilon$ 以上になることを示す.

%     まず, $\varepsilon$ に対して, $1 / M^2 < \varepsilon / 2$ となるような $M$ を取り, $\sigma_{\mathcal{ALG}}^M$ を構成する. 
    
%     Lemma \ref{lmm:all_1_exist_nstar} の仮定が成り立つとき, Lemma \ref{lmm:all_1_exist_nstar} で定義した $n^*$ を取る. すると, $\sigma_{\mathcal{ALG}}^{M, n^* - 1}$ に対するコストの比は, 
%     \[
%         1 + \frac{M^2 - 1}{M^2} = 2 - \frac{M^2 - 1}{M^2} > 2 - \varepsilon
%     \]
%     より競合比は $2 - \varepsilon$ 以上になる.

%     Lemma \ref{lmm:all_1_no_exist} の仮定が成り立つとき, 任意の $2$ 以上の整数 $n$ について, $\sigma_{\mathcal{ALG}}^{M, n}$ に対するコストの比は,
%     \[
%         \frac{n - 1}{n} + \frac{M^2 - 1}{M^2}
%     \]
%     以上である. よって, $1 / n' < \varepsilon / 2$ を満たす $n'$ を取ると, $\sigma_{\mathcal{ALG}}^{M, n'}$ に対するコストの比は, 
%     \[
%         \frac{n' - 1}{n'} + \frac{M^2 - 1}{M^2} = 2 - \frac{1}{n'} - \frac{M^2 - 1}{M^2} > 2 - \varepsilon
%     \]
%     以上となる. 

%     したがって, 任意のオンラインアルゴリズムと任意の $\varepsilon > 0$ について, 競合比は $2 - \varepsilon$ 以上である. 
% \end{proof}

==> figures/flow_chart_recurring.tex <==
\begin{tikzpicture}[scale=0.95, every node/.style={scale=0.95, inner sep=1pt}]
% \begin{tikzpicture}
    \tikzset{Terminal/.style={rounded rectangle, draw, text centered, text width=6cm, minimum height=.5cm, inner sep=1mm}};
    \tikzset{Process/.style={rectangle,  draw,  text centered, text width=6cm, minimum height=.5cm, inner sep=1mm}};
    \tikzset{Decision/.style={diamond,  draw,  text centered, aspect=4, text width=4.5cm, minimum height=.5cm, inner sep=1mm}};

    \node[Terminal] (s) at (0, 0) {$\textbf{recurring}([p, q], l)$ \\  Let $L \coloneqq |[p, q]|$.};
    % $\overline{a} = \overline{p}$ holds.

    \node[Decision, below=1.1 of s.center] (d1) {$L \leq \alpha$ or $l \geq \alpha$};
    \draw[->, thick] (s) -- (d1);

    \coordinate[right=of d1] (r_d1);

    \node[Terminal, right=1.5 of d1] (c1) {\textbf{return}};
    \draw[->, thick] (d1) -- (c1) node[above, pos=0.5]{Yes};

    \node[Process, below=1.5 of d1.center] (p1) {\textbf{wait} until $W_{\overline{a}}$ increases by $2$};
    \draw[->, thick] (d1) -- (p1) node[left, pos=0.5]{No};
    \node at (p1.north east) [above left] {cost: $2$};
    

    \node[Decision, below=1.1 of p1.center] (d2) {$W_i \geq \frac{l + 1}{\alpha}$ for all $i \in [p, q]$};
    \draw[->, thick] (p1) -- (d2);

    \node[Process, text width=6cm, below=1.5 of d2.center] (p2) {Let $[p', q']$ as a minimal cyclic interval \\ where $W_i \geq (l + 1) / \alpha$ for all $i \notin [p', q']$ \\ \textbf{wait} until $\overline{s} \notin [p, p' - 1]$ \\or $W_p$ increases by $1$};
    \draw[->, thick] (d2) -- (p2) node[left, pos=0.5]{No};

    \node[Terminal] (c2) at ($(c1|-d2)$) {\textbf{call} $\textbf{recurring}([p, q], l + 1)$};
    \draw[->, thick] (d2) -- (c2) node[above, pos=0.5]{Yes} ;

    % \node[Process, text width=6cm, below=1.25 of p2.center] (p2') {\textbf{wait} until $\overline{s} \notin [p, p' - 1]$ \\or $W_p$ increases by $1$};
    % \draw[->, thick] (p2) -- (p2');
    % \node at (p2'.north east) [above left] { cost: $\leq 1$ };

    \node[Decision, below=1.4 of p2.center] (d3) {$W_p$ increased by $1$ in (p2)};
    \draw[->, thick] (p2) -- (d3);

    \node[Terminal] (c3) at ($(c2|-d3)$) {\textbf{call} $\textbf{recurring}([p, q], l + 1)$};
    \draw[->, thick] (d3) -- (c3) node[above, pos=0.5]{Yes};

    \node[Process, below=1.5 of d3.center] (p3) {\textbf{match} $\overline{p' - a}$ requests, then\\ \textbf{wait} until $W_{\overline{a}}$ increases by 2};
    \draw[->, thick] (d3) -- (p3) node[left, pos=0.5]{No};
    \node at (p3.north east) [above left] {cost: $3$};

    \node[Decision, below=1.1 of p3.center] (d4) {$W_i \geq \frac{l+1}{\alpha}$ for all $i \in [p', q']$};
    \draw[->, thick] (p3) -- (d4);

    \node[Process, below=1.5 of d4.center] (p6) {Let $r \coloneqq \argmin_{i \in \{p' + \lfloor 2L / \alpha \rfloor, q\}} \overline{i - p'}$};
    \draw[->, thick] (d4) -- (p6) node[left, pos=0.5]{No};

    \node[Process] (p4) at ($(c2|-d4)$) {\textbf{wait} until $\overline{s} \notin [p', p - 1]$ or $W_{p'}$ increases by $1$};
    \draw[->, thick] (d4) -- (p4) node[above, pos=0.5]{Yes};
    \node at (p4.north east) [above left] {cost: $\leq 1$};

    \node[Process, below=1.5 of p4.center] (p5)  {if $\overline{s} \in [p, p' - 1]$ then \textbf{match} $\overline{p - a}$ requests};
    \draw[->, thick] (p4) -- (p5);
    \node at (p5.north east) [above left] {cost: $\leq 1$};
    
    \node[Terminal, below=1.25 of p5.center] (c5) {\textbf{call} $\textbf{recurring}([a, q], l + 1)$};
    \draw[->, thick] (p5) -- (c5);

    % ($(A|-B)!(B|-A)!(B|-B)$)
    \node[Terminal] (c4) at ($(p6|-c5)$) {\textbf{call} $\textbf{recurring}([p', r], l)$};
    \draw[->, thick] (p6) -- (c4);

    % \coordinate[right=of c5] (r_of_c5);
    % \draw[->, thick] (d1) -| (r_of_c5) node[above, pos=0.05]{Yes} -- (c5);

    % \draw[->, thick] (d2) -| (r_of_c5) node[above, pos=0.05]{Yes} -- (c5);

    % Labels
    \node (p1_label) at (p1.north west) [above right] {(p1)};
    \node at ($(d1.north west-|p1_label)$) {(d1)};
    \node at ($(d2.north west-|p1_label)$) {(d2)};
    \node at (p2.north west) [above right] {(p2)};
    % \node at (p2'.north west) [above right] {(p3)};
    \node at ($(d3.north west-|p1_label)$) {(d3)};
    \node at (p3.north west) [above right] {(p3)};
    \node at ($(d4.north west-|p1_label)$) {(d4)};
    \node at (p6.north west) [above right] {(p6)};
    \node at ($(c4.north west-|p1_label)$) [above] {(c5)};

    
    \node (p4_label) at (p4.north west) [above right] {(p4)};
    \node at (p5.north west) [above right] {(p5)};
    \node at ($(c1.north west-|p4_label)$) [above] {(c1)};
    \node at ($(c2.north west-|p4_label)$) [above] {(c2)};
    \node at ($(c3.north west-|p4_label)$) [above] {(c3)};
    \node at ($(c5.north west-|p4_label)$) [above] {(c4)};
\end{tikzpicture}



==> figures/lemma_interval_figure.tex <==
\begin{minipage}{.47\textwidth}
\centering
\begin{tikzpicture}[scale=.6,font=\small]
    % Define the points
    \coordinate (p) at (1,0);
    \coordinate (i) at (8,0);
    \coordinate (q) at (9,0);
    \coordinate (r) at (2,0);

    % Draw the segments
    \draw[blue, thick, fill=blue!10, transform canvas={xshift=-.5pt}] (10,0) -- (i) -- ++(0,0.5) -- (10, 0.5);
    \draw[blue, thick, fill=blue!10] (0,0.5) -- ($(r)+(0,0.5)$) node[midway, above] {(ii)} -- (r) -- (0,0);
    \draw[red,thick,fill=red!10] (10,0) -- (i) -- ++(0,0.3) -- (10,0.3) node[midway, above=.2] {(i)};
    \draw[red,thick,fill=red!10] (0, 0.3) -- ($(p)+(-0.5,0.3)$) -- (p) -- (0,0);

    % Draw the number line
    \draw[very thick] (-0.1,0) -- (10.1,0);
    \foreach \x in {0,0.5,...,10} \draw[very thin] (\x,.1) -- (\x,-.1);
    \node[below] at (10.3,0) {$\mathbb{Z}_k$};

    % Draw the points
    \fill (p) circle (3pt) node[below] {$p$};
    \fill (i) circle (3pt) node[below] {$i$};
    \fill (q) circle (3pt) node[below] {$q$};
    \fill (r) circle (3pt) node[below=0.1, xshift=30, scale=.8] {$\overline{i {+} \left\lceil (\overline{i-p})/(\alpha - 1)\right\rceil {-} 1}$};
\end{tikzpicture}
\subcaption{$\gamma=\overline{p-i}$} \label{subfig:gamma_overpass_p}
\end{minipage}%
\begin{minipage}{.06\textwidth}\mbox{}\end{minipage}%
\begin{minipage}{.47\textwidth}
\centering
\begin{tikzpicture}[scale=.6,font=\small]
    % Define the points
    \coordinate (p) at (1,0);
    \coordinate (i) at (3,0);
    \coordinate (q) at (9,0);
    \coordinate (r) at (4.5,0);

    % Draw the segments
    \draw[red,thick,fill=red!10] (10,0) -- (i) -- ++(0,0.3) -- (10,0.3) node[midway, above] {(i)};
    \draw[red,thick,fill=red!10] (0, 0.3) -- ($(p)+(-0.5,0.3)$) -- (p) -- (0,0);
    
    \draw[blue, thick, fill=blue!12.5, fill opacity=.8, transform canvas={xshift=.3pt}] (i) -- ++(0,0.5) -- ($(r)+(0,0.5)$) node[midway, above, opacity=1] {(ii)} -- (r) -- (i);

    % Draw the number line
    \draw[very thick] (-0.1,0) -- (10.1,0);
    \foreach \x in {0,0.5,...,10} \draw[very thin] (\x,.1) -- (\x,-.1);
    \node[below] at (10.3,0) {$\mathbb{Z}_k$};

    % Draw the points
    \fill (p) circle (3pt) node[below] {$p$}; % [fill=white,draw=black,thick]
    \fill (i) circle (3pt) node[below] {$i$};
    \fill (q) circle (3pt) node[below] {$q$};
    \fill (r) circle (3pt) node[below=0.1, xshift=20, scale=.8] {$\overline{i {+} \left\lceil (\overline{i-p})/(\alpha - 1)\right\rceil {-} 1}$};
\end{tikzpicture}
\subcaption{$\gamma=\big\lceil (\overline{i - p})/(\alpha - 1) \big\rceil$} \label{subfig:gamma_below_p}
\end{minipage}%
\begin{comment}
\begin{tikzpicture}
    % Draw the number line
    \draw[->] (0,0) -- (10,0);

    % Define the points
    \coordinate (q) at (0.5,0);
    \coordinate (p) at (1.5,0);
    \coordinate (i) at (9.5,0);
    \coordinate (r) at (3, 0);

    % Draw the segments
    \draw[red,thick] (i) -- ++(0,0.2) -- (10,0.2);
    \draw[red, thick] (0, 0.2) -- ($(p) + (0, 0.2)$) node[midway, above] {(1)} -- ++(0, -0.2);
    
    \draw[blue, thick] (i) -- ++(0,-0.15) -- (10, -0.15);
    \draw[blue, thick] (0, -0.15) -- (3, -0.15) node[pos=0.8, below] {(2)} -- ++(0, 0.15);

    % Draw the points
    \fill (p) circle (2pt) node[below=0.1cm] {$p$};
    \fill (i) circle (2pt) node[below=0.1cm] {$i$};
    \fill (q) circle (2pt) node[below=0.1cm] {$q$};

    % Draw the arrows to show the cycle
\end{tikzpicture}


\begin{tikzpicture}
    % Define the points
    \coordinate (i) at (1,0);
    \coordinate (q) at (3,0);
    \coordinate (p) at (7,0);
    \coordinate (r) at (6.3,0);

    % Draw the segments
    \draw[red,thick,fill=red!10] (i) -- ++(0,0.2) -- ($(p)+(0,0.2)$) node[midway, above] {(1)} -- ++(0,-0.2);    
    \draw[blue, thick, fill=blue, fill opacity=.1] (i) -- ++(0,-0.2) -- ($(r)+(0,-.2)$) node[midway, above, opacity=1] {(2)} -- ++(0, 0.2) -- (i);

    % Draw the points
    \fill (p) circle (2pt) node[below] {$p$};
    \fill (i) circle (2pt) node[below] {$i$};
    \fill (q) circle (2pt) node[below] {$q$};
    \fill (r) circle (2pt) node[below=2mm] {$i + \left\lceil \frac{\overline{i-p}}{\alpha - 1}\right\rceil - 1$};

    % Draw the number line
    \draw[->, thick] (0,0) -- (10,0);


    % Draw the arrows to show the cycle
\end{tikzpicture}
\end{comment}
